Force Map: Learning to Predict Contact Force Distribution from Vision

When humans see a scene, they can roughly imagine the forces applied to objects based on their experience and use them to handle the objects properly. This paper considers transferring this "force-visualization" ability to robots. We hypothesize that a rough force distribution (named "force map") can be utilized for object manipulation strategies even if accurate force estimation is impossible. Based on this hypothesis, we propose a training method to predict the force map from vision. To investigate this hypothesis, we generated scenes where objects were stacked in bulk through simulation and trained a model to predict the contact force from a single image. We further applied domain randomization to make the trained model function on real images. The experimental results showed that the model trained using only synthetic images could predict approximate patterns representing the contact areas of the objects even for real images. Then, we designed a simple algorithm to plan a lifting direction using the predicted force distribution. We confirmed that using the predicted force distribution contributes to finding natural lifting directions for typical real-world scenes. Furthermore, the evaluation through simulations showed that the disturbance caused to surrounding objects was reduced by 26 % (translation displacement) and by 39 % (angular displacement) for scenes where objects were overlapping.

==> force from vision/related_work.tex <==
% visionからforceを推定する研究は多くあるが，人の身体とのinteractionにfocusしたものが多い．
% 物体操作時にhuman handが物体に加えるcontact forceの推定\cite{Ehsani2020UseTF}\cite{8085141}\cite{Pham2015TowardsFS}，
% 人の身体と物体のinteraction forceの推定\cite{Zhu2016InferringFA}\cite{Li2019Estimating3M}などがある．
% robotがgripperでobjectに力を加える状況を想定したinteraction forceの推定\cite{Shin2018SequentialIA}\cite{Hwang2017InferringIF}，
% deformable objectが多数の点で別の物体に接触する場合のinteraction forceの推定\cite{Wang2022VisualHR}も行われている．
% しかし，我々の知る限り複数物体がinteractionをするstaticなsceneを対象として，visionからcontact forceの推定を行った研究はない．

Several previous works have explored force estimation from vision, but most of them focus on interactions between objects and a human: the contact force applied by the human hand to an object during object manipulation~\cite{Ehsani2020UseTF}\cite{8085141}\cite{Pham2015TowardsFS} or
the interaction force between objects and human bodies~\cite{Zhu2016InferringFA}\cite{Li2019Estimating3M}.
The estimation of the interaction force applied to objects assuming a situation 
where a robot gripper applies force to them~\cite{Shin2018SequentialIA}\cite{Hwang2017InferringIF} and
the estimation of the interaction force applied when a deformable object contacts another object at many contact points~\cite{Wang2022VisualHR}, have also been performed.
However, to the best of our knowledge, there has been no study on the estimation of contact force from the vision for a static scene with multiple objects interacting with each other.

% 本論文が扱うのはこのようなstaticなsceneが与えられた時に，物体の接触によって生じるcontact forceの推定を行う問題である．
% visionからphysical reasoning of objectsを行うhuman cognitive abilityはintrinsic physicsと呼ばれ，deep learningの発展と合わせて研究が進んでいる\cite{Duan2022ASO}.
% staticなsceneを対象としたphysical reasoningで代表的なタスクはstability prediction\cite{Lerer2016LearningPI}\cite{Groth2018ShapeStacksLV}である．
% 多様な形状の物体が積まれたシーンに対する安定性の判断，不安定な場所をheatmapで表現，physical-interactionのoutcomeの予測などが行われている．
% しかし，これらのstudyは直接にinteraction forceを予測するものではない．
% またmass densityの一様性などphysical propertyに関する前提は多様な物品が積まれたシーンに
% そのまま適用することはできない．
This paper deals with the problem of estimating the interaction force between a group of objects stacked according to gravity.
Thus, this is a kind of scene-understanding problem.
The human cognitive ability to perform physical reasoning of objects from vision is called intrinsic physics, which has been studied in conjunction with the advancement of machine learning~\cite{Duan2022ASO}.
A typical task in physical reasoning for a static scene is stability prediction~\cite{Lerer2016LearningPI}\cite{Groth2018ShapeStacksLV}.
These works include determining the stability of a scene with objects of various shapes stacked on top of each other, 
predicting the point of stability as a heat-map, and predicting the outcome of physical interactions.
However, these works do not directly predict the interaction force.
Also, assumptions about physical properties, such as the uniformity of mass density, cannot be applied directly to a scene with various kinds of objects.

% 視覚からinteraction forceを推定するには，forceと相関がある視覚情報の存在が必要となる．
% 上で挙げた研究もその多くが物体の動き[][][]や変形[][][]といったforceと相関がある視覚情報を利用している．
% 人が力を加える場合には加えて生体ならではのappearanceの変化も利用できる\cite{Grady2023VisualEO}．
% しかし，変形が観測できない程度に小さい物体が積まれたstaticなsceneについてはこれらの手がかりは使えない．
% したがって，物体の質量など物体固有の情報を視覚から予測する必要がある．
% introductionで説明したように我々は物体種類あるいは物体のappearanceとこれらのphysical propertyに統計的に相関があると仮定する．
% このような仮定は高精度の推定には不十分でも大まかな推論には使える場合がある．
% computer visionではappearanceからmaterialやtextureの推論はcommonである．
% appearanceからtactile propertyの推定\cite{Takahashi2018DeepVL}，
% stiffnessの推定\cite{doi:10.1080/01691864.2022.2078669}もexplored．
% 我々はappearanceからphysical interactionの結果として生じる力の分布をend-to-endで学習させる．
% massなどを陽に推定するわけではないが，物体のappearanceからinternallyに推定しているとみなすことができる．
% ただし，高精度で行うことを目指すのでなく，大まかな分布という形で 推定することでrobotのタスクに有用な情報を予測することを目指す．
Visual information correlated with the force is necessary to estimate interaction force from vision.
Many of the above-mentioned studies use the movement~\cite{Ehsani2020UseTF}\cite{8085141}\cite{Pham2015TowardsFS}\cite{Li2019Estimating3M}
and/or deformation~\cite{Zhu2016InferringFA}\cite{Shin2018SequentialIA}\cite{Hwang2017InferringIF}\cite{Wang2022VisualHR}
as such visual cues.
% When a human applies force, biomechanical properties that cause appearance change can also be utilized~\cite{Grady2023VisualEO}.
However, these cues are unavailable for static scenes with no observable deformation.
Therefore, as explained in the introduction, we assume a statistical correlation between object type, appearance, and physical properties such as mass.
Such an assumption may not be sufficient for highly accurate estimation, but it can be utilized for rough inference.
In computer vision, inferring properties such as material and texture from appearance is common~\cite{Xiao2018UnifiedPP}. 
In robotics, the estimation of tactile properties~\cite{Takahashi2018DeepVL} and
stiffness~\cite{doi:10.1080/01691864.2022.2078669} from vision have been explored.
Our approach is end-to-end learning from appearance to physical interactions.
Although this approach does not explicitly estimate the properties such as mass, 
it is thought to correlate the appearance of objects to physical properties internally.

% works on physical inference of humans
% \cite{doi:10.1073/pnas.1306572110}\cite{li_wang_boger_smith_gershman_ullman_2022}

The essential part of the proposed method is generating
contact force information caused by contact between multiple
objects by simulation and using it for training. 
This sensory information is usually unavailable in reality. % is called privileged information and
Such approaches are particularly effective in predicting information
that cannot be measured in the real world, such as the depth
of transparent objects~\cite{Sajjan2019ClearG3}. 
Such information is also utilized for the motion generation of robots~\cite{Lee2020LearningQL}. 
Although these approaches aim to obtain models
applicable to real-world input, it does not necessarily
mean that making the simulation close to reality is essential. 
Lee et al. trained the controller of a quadruped robot
using only rigid terrains and a small set of procedurally
generated terrains. However, the controller handled complex
real terrains, including deformable terrains~\cite{Lee2020LearningQL}. 
We also use a general-purpose simulator in which objects are modeled
as rigid bodies, and the geometries of objects are simplified but
we expect the trained model works for real scenes.

% There are a variety of applications to train a model applicable to the real world by utilizing this kind of information obtained in simulation.
% In robot learning, this kind of information, which is called privileged information, has been utilized.
% In reinforcement learning and imitation learning that use images as input, they often use the privileged information as sub-tasks to learn latent representations suitable for each task~\cite{Kase2020TransferableTE}.

% Newtonian Image Understanding
% Contact DB

% Our training in simulation only uses rigid terrains and a small set of procedurally generated terrain profiles, such as hills and steps. However, when deployed on physical quadrupeds, the controller successfully handled deformable terrains (mud, moss, and snow); dynamic footholds (stepping on a rolling board in a cluttered indoor environment or debris in the field); and overground impediments such as thick vegetation, rubble, and gushing water. Our methodology may lead to future developments for legged robotics. Moreover, our results suggest that the extraordinary complexity of the physical world can be tamed without brittle and painstaking modeling or dangerous and expensive trial and error under real-world field conditions.
